V-Doc : Visual questions answers with Documents

We propose V-Doc, a question-answering tool using document images and PDF, mainly for researchers and general non-deep learning experts looking to generate, process, and understand the document visual question answering tasks. The V-Doc supports generating and using both extractive and abstractive question-answer pairs using documents images. The extractive QA selects a subset of tokens or phrases from the document contents to predict the answers, while the abstractive QA recognises the language in the content and generates the answer based on the trained model. Both aspects are crucial to understanding the documents, especially in an image format. We include a detailed scenario of question generation for the abstractive QA task. V-Doc supports a wide range of datasets and models, and is highly extensible through a declarative, framework-agnostic platform.

==> others.tex <==
\begin{table*}[t!]
    \caption{Existing Datasets in Dataset Library}
    \label{tab:dataset}
    \centering
    \begin{tabular}{lllll}
    \toprule
    \textbf{Dataset} & \textbf{Image Source} & \textbf{Answer Type} & \textbf{Num of Images} & \textbf{Num of QA pairs} \\ \midrule
    FUNSD & Forms & Extractive & 199 & \\
    DocVQA & Single page documents & Extractive & 12K & 50K \\
    \midrule
    Clevr & Synthetic images & Abstractive & 100K & 865K \\
    Ours & Medical academic papers & Abstractive & & \\
    \endrule
    \end{tabular}
\end{table*}
